Model-Free Assortment Pricing with Transaction Data

We study the problem when a firm sets prices for products based on the transaction data, i.e., which product past customers chose from an assortment and what were the historical prices that they observed. Our approach does not impose a model on the distribution of the customers' valuations and only assumes, instead, that purchase choices satisfy incentive-compatible constraints. The individual valuation of each past customer can then be encoded as a polyhedral set, and our approach maximizes the worst-case revenue assuming that new customers' valuations are drawn from the empirical distribution implied by the collection of such polyhedra. We show that the optimal prices in this setting can be approximated at any arbitrary precision by solving a compact mixed-integer linear program. Moreover, we study the single-product case and relate it to the traditional model-based approach. We also design three approximation strategies that are of low computational complexity and interpretable. Comprehensive numerical studies based on synthetic and real data suggest that our pricing approach is uniquely beneficial when the historical data has a limited size or is susceptible to model misspecification.

==> Data Driven Assortment Pricing(1)/dook.tex <==
n	value   error	value2	error2  value3  error3  value4  error4
20	.086    .018    .093    .018    .088    .015    0.106   .016
30	.051    .016    .059    .016    .097    .018    .111    .018
40	.031    .014    .039    .014    .091    .018    .103    .018
50  .053    .017    .06     .017    .097    .018    .107    .018
60	.03     .015    .036    .015    .068    .017    .078    .017
70	.004    .014    .009    .013    .123    .021    .133    .021
80	-.001   .012    .003    .012    .083    .018    .09     .018
90	-.013   .011    -.009   .011    .062    .017    .07     .017
100 -.013   .01     -.01    .01     .056    .016    .064    .016
110 -.027   .007    -.024   .007    .073    .018    .08     .018









==> dook.tex <==
n	value   error	value2	error2  value3  error3  value4  error4
20	.086    .018    .093    .018    .088    .015    0.106   .016
30	.051    .016    .059    .016    .097    .018    .111    .018
40	.031    .014    .039    .014    .091    .018    .103    .018
50  .053    .017    .06     .017    .097    .018    .107    .018
60	.03     .015    .036    .015    .068    .017    .078    .017
70	.004    .014    .009    .013    .123    .021    .133    .021
80	-.001   .012    .003    .012    .083    .018    .09     .018
90	-.013   .011    -.009   .011    .062    .017    .07     .017
100 -.013   .01     -.01    .01     .056    .016    .064    .016
110 -.027   .007    -.024   .007    .073    .018    .08     .018








